uniINF: Best-of-Both-Worlds Algorithm for Parameter-Free Heavy-Tailed MABs

In this paper, we present a novel algorithm, uniINF, for the Heavy-Tailed Multi-Armed Bandits (HTMAB) problem, demonstrating robustness and adaptability in both stochastic and adversarial environments. Unlike the stochastic MAB setting where loss distributions are stationary with time, our study extends to the adversarial setup, where losses are generated from heavy-tailed distributions that depend on both arms and time. Our novel algorithm `uniINF` enjoys the so-called Best-of-Both-Worlds (BoBW) property, performing optimally in both stochastic and adversarial environments without knowing the exact environment type. Moreover, our algorithm also possesses a Parameter-Free feature, i.e., it operates without the need of knowing the heavy-tail parameters $(\sigma, \alpha)$ a-priori. To be precise, uniINF ensures nearly-optimal regret in both stochastic and adversarial environments, matching the corresponding lower bounds when $(\sigma, \alpha)$ is known (up to logarithmic factors). To our knowledge, uniINF is the first parameter-free algorithm to achieve the BoBW property for the heavy-tailed MAB problem. Technically, we develop innovative techniques to achieve BoBW guarantees for Parameter-Free HTMABs, including a refined analysis for the dynamics of log-barrier, an auto-balancing learning rate scheduling scheme, an adaptive skipping-clipping loss tuning technique, and a stopping-time analysis for logarithmic regret.

==> DRAFT.tex <==

\section{Below is draft}
\subsection{The Analysis of Skipping Error}
\label{sec:regret-skipping}
To control the skipping error, we first define $h_t := \ell_{t,i_t} - \ell_{t,i_t}^{\text{skip}}$ as the loss of clipping operation, and $\textsc{SkipErr}_t$ as the single step skipping error for $t \in [T]$, \textit{i.e.},
$$ \textsc{SkipErr}_t := \langle \vx_t - \vy, \vl_t - \vl^{\text{skip}}_t \rangle. $$

Then we have
\begin{align*}
    \textsc{SkipErr}_t
    & = \sum_{i \in [K]} (x_{t,i} - y_i) \cdot (\ell_{t,i} - \ell_{t,i}^{\text{skip}}) \\ 
    & \leq  \sum_{i\ne i^\ast} x_{t,i} \cdot \left|\ell_{t,i} - \ell^{\text{skip}}_{t,i}\right| + (x_{t,i^\ast} - 1) \cdot \left(\ell_{t,i^\ast} - \ell_{t,i^\ast}^{\text{skip}}\right).
\end{align*}


We aim to control the expectation of $\textsc{SkipErr}_t$. For the second term, the factor $x_{t,i^\ast} - 1$ is $\mathcal F_{t-1}$-measurable, and we have 
\begin{align*}
    \E\left[\ell_{t,i^\ast} - \ell_{t,i^\ast}^{\text{skip}} \middle| \mathcal F_{t-1}\right] & = \E\left[\mathbbm{1}[\lvert \ell_{t,i^\ast} \rvert \geq C_{t,i^\ast}]\cdot \ell_{t,i^\ast} \right]  \ge 0
\end{align*}
where the inequality is due to the truncated non-negative assumption (\Cref{ass:truncated-non-negative}) of the optimal arm $i^\ast$.


Therefore, we have $\mathbb E[(x_{t,i^\ast} - 1) \cdot (\ell_{t,i^\ast} - \ell_{t,i^\ast}^{\text{skip}})\mid \mathcal F_{t-1}] \le 0$ and
\begin{align}
\label{eq:Bt-bound-by-ht}
    \mathbb E[\textsc{SkipErr}_t\mid \mathcal F_{t-1}] & \leq  \mathbb E[\lvert h_t \rvert \cdot \mathbbm{1}[i_t \ne i^\ast] \mid \mathcal F_{t-1}].
\end{align}

\yu{Next we need to briefly introduce how to bound the }

\subsection{The Analysis of Main Regret}
\label{sec:regret-ftrl}

By FTRL regret decomposition \yu{todo, add this decomposition lemma's detailed proof}, we have
\begin{align*}
    \textsc{FTRL} &= \E\left[ \sum_{t = 1}^T \langle \vx_t - \wt\vy , \vl^{\text{skip}}_t \rangle \right] = \E\left[ \sum_{t = 1}^T \langle \vx_t - \wt\vy , \wt{\vl}_t \rangle \right] \\
    &\leq \sum_{t=1}^T  \E[D_{\Psi_t}(\vx_t, \vz_t)] + \E[(\Psi_{t+1} - \Psi_{t})(\tilde \vy) - (\Psi_{t+1} - \Psi_{t})(\vx_t)].
\end{align*}

We further denote the per-round \textsc{FTRL} error as
\begin{align*}
    \textsc{FTRL}_t := D_{\Psi_t}(\vx_t, \vz_t) + (\Psi_t - \Psi_{t-1})(\tilde \vy) - (\Psi_t - \Psi_{t-1})(\vx_t),
\end{align*}
where
\begin{align}
    &\vx_t := \argmin_{\vx \in \Delta^{[K]}} - \langle \mL_{t-1}, \vx\rangle + \Psi_t(\vx), \\
    &\vz_t := \argmin_{\vz \in \Delta^{[K]}} -\langle \mL_t, \vz \rangle + \Psi_t(\vz).
\end{align}
and $\mL_t$ is the cumulative loss
\begin{align*}
    \mL_t = \sum_{s=1}^t \wt{\vl}_s.
\end{align*}

By KKT conditions, there exist two unique scalars $Z_t$ and $\wt{Z}_t$ such that
\begin{align*}
    x_{t,i} = \frac{S_t}{L_{t-1,i} - Z_t}, \quad z_{t,i} = \frac{S_t}{L_{t,i} - \wt{Z}_t},\quad \forall i\in [K].
\end{align*}





\subsubsection{The Bregman Divergence Term}
First we analyze the Bregman divergence term. We denote $\textsc{Div}_t := D_{\Psi_t}(\vx_t, \vz_t)$ as the Bregman divergence between $\vx_t$ and $\vz_t$ under regularizer $\Psi_t$, and $\textsc{Shift}_t := (\Psi_t - \Psi_{t-1})(\wt \vy) - (\Psi_t - \Psi_{t-1})(\vx_t)$ as the $\Psi$-shift term.

By definition of $\Psi_t$ in \Cref{eq:Psi-def}, we have
\begin{align*}
    \nabla \Psi_t (\vz_t) = \left[ -\frac{S_t}{z_{t,i}} : {i\in[K]}\right],
\end{align*}
and thus
\begin{align*}
    \textsc{Div}_t &= \Psi_t(\vx_t) - \Psi_t(\vz_t) - \langle \nabla\Psi_t(\vz_t) , \vx_t - \vz_t\rangle \\
    &= S_t\sum_{i\in[K]}\left (-\log \frac{x_{t,i}}{z_{t,i}} + \frac{x_{t,i}}{z_{t,i}} - 1\right ). 
\end{align*}
Denote 
\begin{align*}
    w_{t,i} := \frac{x_{t,i}}{z_{t,i}} - 1 = \frac{L_{t,i} - \wt{Z}_t}{L_{t-1,i} - {Z}_t} - 1 = \frac{\wt{\ell}_{t,i} - (\wt{Z}_t - Z_t)}{L_{t-1,i} - Z_t}.
\end{align*}
Then we have
\begin{align*}
    \textsc{Div}_t = S_t \sum_{i\in[K]} w_{t,i} - \log(w_{t,i} + 1).
\end{align*}

One directly idea is applying the inequality $x - \log(x + 1) \leq x^2$ for $x\in[-1/2, 1/2]$. Then, we use the following lemma to show $w_{t,i} \in [-1/2, 1/2]$, \textit{i.e.}, $\frac{1}{2}x_{t,i} \leq z_{t,i} \leq 2x_{t,i}$.


By inspecting the partial derivatives of the multiplier $\tilde Z_t$ with respect to the feedback vector $\tilde \vl_t$, we can derive the following lemmas on $w_{t,i}$.
\begin{lemma}
% \label{lemma:w-expression}
We have
\begin{align*}
    w_{t,i} = \wt \ell_{t,i_t} \cdot \frac{x_{t,i}}{S_{t}} \cdot \left(\mathbbm{1} [i=i_t] - \frac{{\zeta_{t,i_t}^2}} {\sum_{k\in[K]}{\zeta_{t,k}^2}}\right),
\end{align*}
where
\begin{align*}
    \zeta_t := \argmin_{\vz \in \Delta} -\langle \mL_{t-1} + \lambda \tilde \ell_t, \vz \rangle + \Psi_t(\vz).
\end{align*}
Here $\lambda$ is some constant ranged from $(0,1)$, implicitly determined by $\tilde \ell_t$.
\begin{proof}
    Notice that conditioning on the time step before $t - 1$, $z_{t,i}$ only depends on $\wt{\ell}_{t,i}$. Then we denote
    \begin{align*}
        \wt{Z}'_{t,i}(\theta):=\left.\frac{\partial \tilde Z_t}{\partial \wt{\ell}_{t,i}}\right\vert_{\wt{\vl}_{t} = \theta\ve_i},
    \end{align*}
    where $\ve_i$ is the unit vector supported at the $i$-th coordinate, and $\theta$ is a scalar.
    
    Notice that 
    \begin{align}
        \sum_{j\in[K]} z_{t,j} = \sum_{j\in[K]} \frac{S_t}{L_{t,j} - \wt{Z}_t} = 1, \label{eq:z-sum-to-1}
    \end{align}
    Then partially derivate $\wt{\ell}_{t,i}$ on both sides of \Cref{eq:z-sum-to-1}, we get
    \begin{align*}
        \sum_{j\in[K]} -\frac{S_{t}}{(\ell_{t,j} - \wt{ Z}_t)^2}\cdot(\mathbbm{1}[j=i] - \wt{Z}'_{t,i}) = - \frac{z_{t,i}^2}{S_{t}} +  \wt{Z}_{t,i}^{\text{skip}} \sum_{j\in[K]}
        \frac{z_{t,j}^2}{S_{t}} = 0,
    \end{align*}
    which solves to 
    \begin{align*}
        \wt{Z}'_{t,i} = \frac{z_{t,i}^2}{\sum_{j\in[K]} {z_{t,j}^2}}.
    \end{align*}
    
    Similarly, we denote
    \begin{align*}
        z'_{t,ij}(\theta) := \left.\frac{\partial z_{t,i}}{\partial \wt \ell_{t,j}}\right\vert_{\wt \vl_{t} = \theta \ve_j}
    \end{align*}
    Then according to the chain rule, we have
    \begin{align*}
        z'_{t,ij} = \frac{z_{t,i}^2}{S_{t}} \cdot\left( z_{t,j}^2/ \left(\sum_{k\in[K]}{x_{t,k}^2}\right) - \mathbbm{1}[i=j] \right).
    \end{align*}
    

    We denote
    \begin{align*}
        w'_{t,ij}(\theta) & :=\left.\frac{\partial w_{t,i}}{\partial \wt \ell_{t,j}}\right\vert_{\wt \vl_{t} = \theta \ve_j}.
    \end{align*}
    Recall that $w_{t,i} = \frac{x_{t,i}}{S_{t}}(\tilde \ell_{t,i} - (\tilde Z_t - Z_t))$, hence
    \begin{align*}
        w'_{t,ij} & = \frac{x_{t,i}}{S_{t}}\cdot \left(\mathbbm{1}[i=j] - \left( \frac{z_{t,j}^2}{S_{t}}\right) / \left(\sum_{k\in[K]}\frac{z_{t,k}^2}{S_{t}}\right)\right) \\
        & =\frac{x_{t,i}}{S_{t}}\cdot \left(\mathbbm{1}[i=j] - \left( {z_{t,j}^2}\right) / \left(\sum_{k\in[K]}{z_{t,k}^2}\right)\right).
    \end{align*}

    Thus according to the intermediate value theorem, we have
    \begin{align*}
        w_{t,i} = \wt \ell_{t,i_t} \cdot \frac{x_{t,i}}{S_{t}} \cdot \left(\mathbbm{1} [i=i_t] - \frac{{\zeta_{t,i_t}^2}} {\sum_{k\in[K]}{\zeta_{t,k}^2}}\right),
    \end{align*}
    where
    \begin{align*}
        \zeta_t := \argmin_{\vz \in \Delta^{[K]}} -\langle \mL_{t-1} + \lambda \tilde \ell_t, \vz \rangle + \Psi_t(\vz),
    \end{align*}
    and $\lambda$ is some constant ranged from $(0,1)$, implicitly determined by $\tilde \ell_t$. Furthermore, \Cref{lemma:constantly-apart} guarantees that
    \begin{align*}
        x_{t,i} / 2 \le \zeta_{t,i} \le 2x_{t,i} \quad \forall i \in [K]. 
    \end{align*}
\end{proof}
\end{lemma}

Equipped with the uppper bounds of $w_{t,i}^2$, we can then bound $\textsc{Div}_t$ by $\gO(S_{t}^{-1}\cdot (\ell^{\text{skip}}_{t,i_t})^2 \cdot (1 - x_{t,i_t})^2)$.
\begin{lemma}[The Upper Bound of the Bregman Divergence Terms]
% \label{lemma:bregman-bound}
The expectation of the Bregman Divergence term $\textsc{Div}_t$ can be bounded by follows
%\jiatai{change the name of this lemma}
\begin{align*}
    \E[\textsc{Div}_t] \leq 8192 \sum_{i\in[K]}S_t^{-1}\E[(\ell^{\text{skip}}_{t,i})^2]x_{t,i}(1 - x_{t,i})^2,
\end{align*}
which gives that $\textsc{Div}_t = \gO\left( S_t^{-1}(\ell^{\text{skip}}_{t,i_t})^2(1 - x_{t,i_t})^2 \right)$

\begin{proof}
    Recall the definition of $w_{t,i}$, we have
    \begin{align*}
        \E[\textsc{Div}_t] & =\sum_{i \in [K]}\E\left[S_t(w_{t,i} - \log(1 + w_{t,i}))\right]
    \end{align*}
    By \Cref{lemma:constantly-apart}, we have $w_{t,i} = x_{t,i}/z_{t,i} - 1 \in [-1/2, 1/2]$. Therefore, since $x - \log(1 + x) \leq x^2$, we have
    \begin{align*}
        \E[\textsc{Div}_t] \leq \sum_{i\in[K]}S_t\cdot \left(\E[\mathbbm{1}[i=i_t]w_{t,i}^2] + \E[\mathbbm{1}[i\neq i_t]w_{t,i}^2]\right).
    \end{align*}
    By \Cref{lemma:w-expression}, we have
    \begin{align*}
        w_{t,i} = \wt \ell_{t,i_t} \cdot \frac{x_{t,i}}{S_{t}} \cdot \left(\mathbbm{1} [i=i_t] - \frac{{\zeta_{t,i_t}^2}} {\sum_{k\in[K]}{\zeta_{t,k}^2}}\right),
    \end{align*}
    %where $\zeta_t \in \Delta^{[K]}$
    and $\zeta_{t,i}$ satisfying $x_{t,i}/2 \leq \zeta_{t,i} \leq 2x_{t,i}$.
    Then, for $i \neq i_t$, we have
    \begin{align*}
    w_{t,i} & = -\ell^{\text{skip}}_{t,i_t} \cdot \frac{x_{t,i}}{S_{t}} \cdot \frac{\zeta_{t,i_t}}{\sum_{k\in[K]}{\zeta_{t,k}^2}}, \\
    w_{t,i}^2 & = (\ell_{t,i_t}^{\text{skip}})^2 \cdot \frac{x_{t,i}^2}{S_{t}^2} \cdot \frac{\zeta_{t,i_t}^2} {\left(\sum_{k\in[K]}{\zeta_{t,k}^2}\right)^2} \\
    & \le 16 \cdot (\ell_{t,i_t}^{\text{skip}})^2 \cdot \frac{x_{t,i}^2}{S_{t}^2} \cdot \frac{x_{t,i_t}^2} {\left(\sum_{k\in[K]}{x_{t,k}^2}\right)^2}.
    \end{align*}
    And for $i = i_t$,
    \begin{align*}
        w_{t,i} & = \ell^{\text{skip}}_{t,i}\cdot \frac {1} {S_{t}} \cdot  \frac{\sum_{j\ne i} \zeta_{t,j}^2}{\sum_{k\in[K]}{\zeta_{t,k}^2}},\\
        w_{t,i}^2 & = (\ell_{t,i}^{\text{skip}})^2 \cdot \frac{ 1 }{S_{t}^2} \cdot \frac{\left(\sum_{j\ne i} {\zeta_{t,j}^2}\right)^2} { \left(\sum_{k\in[K]}{\zeta_{t,k}^2}\right)^2} \\
        & \le 256\cdot (\ell_{t,i}^{\text{skip}})^2 \cdot \frac{ 1 }{S_{t}^2} \cdot \frac{\left(\sum_{j\ne i} {x_{t,j}^2}\right)^2} { \left(\sum_{k\in[K]}{x_{t,k}^2}\right)^2}.
    \end{align*}
    
    Therefore, we have
    \begin{align*}
        \E[\textsc{Div}_t] &\leq 1024 \sum_{i\in[K]} S_t \cdot   \left( x_{t,i} \E[(\ell_{t,i}^{\text{skip}})^2] \frac{1}{S_t^2}\frac{\left(\sum_{j\ne i} {x_{t,j}^2}\right)^2} { \left(\sum_{k\in[K]}{x_{t,k}^2}\right)^2} 
        + \sum_{j\neq i}x_{t,j}\E[(\ell_{t,j}^{\text{skip}})^2]\frac{x_{t,i}^2}{S_t^2}\frac{x_{t,j}^2} {\left(\sum_{k\in[K]}{x_{t,k}^2}\right)^2}\right) \\
        &= 1024\sum_{i\in[K]} S_t^{-1} \cdot \E[(\ell^{\text{skip}}_{t,i})^2]\cdot \left( x_{t,i} \cdot \left(1 - \frac{x_{t,i}^2}{\sum_{k\in[K] x_{t,k}^2}}\right)^2 + x_{t,i}\cdot \frac{x_{t,i}^2}{\sum_{k\in[K] x_{t,k}^2}} \cdot \sum_{j\neq i}\frac{x_{t,j}^2}{\sum_{k\in[K] x_{t,k}^2}} \right)
    \end{align*}
    \yu{这个地方我好像原本算错了，算完之后好像更好算一些。待验证}\jiatai{感觉没啥问题}\yu{ 请求 一个再次检查 }

    Notice that when $x_{t,i} \leq 1/2$, we have $4(1-x_{t,i})^2 \geq 1$. Then
    \begin{align*}
        &\quad x_{t,i} \cdot \left(1 - \frac{x_{t,i}^2}{\sum_{k\in[K] x_{t,k}^2}}\right)^2 + x_{t,i} \cdot \frac{x_{t,i}^2}{\sum_{k\in[K] x_{t,k}^2}} \cdot \sum_{j\neq i}\frac{x_{t,j}^2}{\sum_{k\in[K] x_{t,k}^2}} \\
        & \le 2x_{t,i} \\
        & \leq 8 x_{t,i} (1 - x_{t,i})^2
    \end{align*}
    trivially holds.
    Then we have
    \begin{align*}
        \E[\textsc{Div}_t] \leq 8192  \sum_{i\in[K]} S_t^{-1} \cdot \E[(\ell^{\text{skip}}_{t,i})^2]\cdot x_{t,i} (1 - x_{t,i})^2.
    \end{align*}

    For $x_{t,i} > 1/2$, we denote
    \begin{align*}
        \wt{x}_{t,i} := \frac{x^2_{t,i}}{\sum_{k\in[K]} x^2_{t,k}},
    \end{align*}
    which directly implies
    \begin{align*}
        \E[\textsc{Div}_t] & \leq1024 \sum_{i\in[K]} S_t^{-1}\E[(\ell_{t,i}^{\text{skip}})^2]\left( x_{t,i}\wt{x}_{t,i}\sum_{j\neq i}\wt{x}_{t,j} + x_{t,i}(1 - \wt{x}_{t,i})^2\right).
    \end{align*}
    Since $x_{t,i} > 1/2$, we have $x_{t,i} \leq \wt{x}_{t,i} \leq 1$ and $\wt{x}_{t,j} \leq x_{t,j}^2 / x_{t,i}^2 \leq 4 x_{t,j}^2$ holds for all $j \neq i$. Therefore, 
    \begin{align*}
        &\quad x_{t,i}\wt{x}_{t,i}\sum_{j\neq i}\wt{x}_{t,j} + x_{t,i}(1 - \wt{x}_{t,i})^2 \\ & \leq x_{t,i} \left( \sum_{j\neq i}4 x_{t,j}^2 + (1 - x_{t,i})^2 \right) \\
        & \leq x_{t,i} \left( 4\left(\sum_{j \neq i} x_{t,j}^2 + 2\sum_{j \neq i, k \neq i, j < k}x_{t,j} x_{t,k}\right) + (1 - x_{t,i})^2 \right) \\
        & \leq5x_{t,i} (1 - x_{t,i})^2,
    \end{align*}
    which gives
    \begin{align*}
        \E[\textsc{Div}_t] \leq 5120 \sum_{i\in[K]} S_t^{-1} \E[(\ell_{t,i}^{\text{skip}})^2]x_{t,i}(1 - x_{t,i})^2.
    \end{align*}
    Then we finish the proof.
\end{proof}
\end{lemma}

\subsubsection{The $\Psi$-shifting Terms}

Besides, for the shifting terms, we have the following lemma.
\begin{lemma}
\label{lemma:shifting-terms}
We can bound the $\Psi$-shifting by the following inequality,
\begin{align*}
    \sum_{t=1}^T \textsc{Shift}_t = \sum_{t=1}^T  \E\left[(\Psi_{t+1} - \Psi_{t})(\tilde \vy) - (\Psi_{t+1} - \Psi_{t})(\vx_t)\right] \leq \E[S_{T+1} \cdot K\log T].
\end{align*}
\begin{proof}
    By definition of $\Psi$ in \Cref{eq:Psi-def} and the summing up telescoping, we have
    \begin{align*}
        &\quad \sum_{t=1}^T  \E[(\Psi_{t+1} - \Psi_{t})(\tilde \vy) - (\Psi_{t+1} - \Psi_{t})(\vx_t)] \\
        &=\sum_{t=1}^T \E\left[ (S_{t+1} - S_t)\cdot \left( \sum_{i\in[K]}\left(-\log(\wt{y}_i) + \log(x_{t,i})\right)\right) \right] \\
        &\leq \sum_{t=1}^T \E\left[ (S_{t+1} - S_t)\cdot \left( \sum_{i\in[K]}\left(-\log(1/T)\right)\right)\right] \\
        &= \sum_{t=1}^T \E\left[ (S_{t+1} - S_t)\cdot K \log T\right] \\
        &= \E[S_{T+1} \cdot K\log T],
    \end{align*}
    where the inequality holds by $(S_{t+1} - S_t) \geq 0$, $\wt{y}_i \geq 1/T$ and $\log(x_{t,i}) \leq 0$. %Then we get the result.
\end{proof}
\end{lemma}

To summarize the bounds of FTRL gap, we have
\begin{equation}
\label{eq:At-bound}
\begin{aligned}
    \E\left[ \sum_{t=1}^T \textsc{FTRL}_t \right] & = \sum_{t=1}^T \E[\textsc{Div}_t] + \sum_{t=1}^T  \E[(\Psi_{t+1} - \Psi_{t})(\tilde \vy) - (\Psi_{t+1} - \Psi_{t})(\vx_t)] \\
    & \leq 8192 \sum_{t=1}^T\sum_{i\in[K]} S_t^{-1} \E\left[(\ell_{t,i}^{\Skip})^2\right] x_{t,i}(1 - x_{t,i})^2 + \E\left[S_{T+1} \cdot K\log T\right].
\end{aligned}
\end{equation}

By previous analyisis,to achieve the theoretical proof of the best of both worlds regret upper bounds for \Cref{alg}, we need to bound the sum of FTRL terms and skipping errors:
\begin{align*}
    \gR_T \leq \E[S_{T+1} \cdot K \log T] + \sum_{t=1}^T \E\left[ |h_t| \cdot \mathbbm{1}[i_t \neq i^\ast] + 8192 S_t^{-1} (\ell_{t,i_t}^{\Skip})^2 (1 - x_{t,i_t})^2 \right].
\end{align*}
We establish the regret analysis for adversarial and stochastic cases separately in following sections.

\section{Adversarial Regret Analysis}
In this section, we prove one of our main results \Cref{thm:regret-adv} for adversarial settings. We consider the upper bounds for three parts, the skipping error $\sum_{t=1}^T \textsc{SkipErr}_t$, the Bregman Divergence terms $\sum_{t=1}^T\textsc{Div}_t$, and $S_{T+1}$ which controls the $\Psi$-shifting gap.
\subsection{The Upper Bound of Bregman Divergence Terms}
We prove that the Bregman Divergence Term can be bounded by the expectation of $S_{T+1}$.
\begin{lemma}
% \label{lemma:adv-bregman}
We have 
\begin{align*}
    \E\left[\sum_{t=1}^T \textsc{Div}_t\right] 
    &\leq 8192(1 + \sqrt{2})\E\left[ S_{T+1} K \log T \right]
\end{align*}
\begin{proof}

Notice that by \Cref{lemma:bregman-bound}, we have
\begin{align*}
    \E\left[\sum_{t=1}^T \textsc{Div}_t\right] \leq \E\left[ 8192\sum_{t=1}^T S_t^{-1} \cdot \left(\ell^{\text{skip}}_{t,i_t}\right)^2 \cdot (1 - x_{t,i_t})^2 \right].
\end{align*}
Notice that by definition of $S_{t+1}$ in \Cref{eq:St-def}, we have
\begin{align*}
    (K \log T)\cdot (S_{t+1}^2 - S_t^2) = \left(\ell^{\text{clip}}_{t,i_t}\right)^2 \cdot (1 - x_{t,i_t})^2.
\end{align*}
Moreover, since $\ell^{\text{clip}}_{t,i_t}$ is controlled by $C_{t,i_t}$, we have
\begin{align}
\label{eq:St+1-upper}
    S_{t+1}^2 \leq S_t^2 + C_{t,i_t}^2 (1 - x_{t,i_t})^2 \cdot (K \log T)^{-1} = S_t^2\left( 1 + (4K \log T)^{-1} \right) \leq 2S_t^2,
\end{align}
where the first inequlity is due to $|\ell^{\text{clip}}_{t,i_t}| \leq C_{t,i_t}$ and the definition of $C_{t,i_t}$ in \Cref{eq:C-def}, and the second inequlity holds by $T \geq 2$.
Therefore, as $\lvert \ell_{t,i_t}^{\text{skip}}\rvert\le \lvert \ell_{t,i_t}^{\text{clip}}\rvert$ trivially, we have
\begin{align*}
    \E\left[\sum_{t=1}^T \textsc{Div}_t\right] &\leq \E\left[8192\sum_{t=1}^T  S_t^{-1} \cdot (\ell^{\text{skip}}_{t,i_t})^2 \left( 1 - {x}_{t,i_t}\right)^2\right] \\
    &\leq 8192\E\left[K\log T\sum_{t=1}^T \frac{S_{t+1}^2 - S_t^2}{S_t}\right] \\
    &= 8192\E\left[K\log T\sum_{t=1}^T \frac{(S_{t+1} + S_t)(S_{t+1} - S_t)}{S_t}\right] \\
    &\leq 8192\E\left[ (1 + \sqrt{2})K\log T \sum_{t=1}^T S_{t+1} - S_t \right] \\
    &= 8192(1 + \sqrt{2})\E\left[ S_{T+1} K \log T \right],
\end{align*}
where the first ineuqality is by \Cref{lemma:bregman-bound}, the second inequality is due to the definition of $S_{t+1}$ in \Cref{eq:St-def} and $|\ell_{t,i_t}^\Skip| \leq |\ell_{t,i_t}^\Clip|$, and the last inequality is due to the $S_{t+1} \leq \sqrt{2} S_t$ by \Cref{eq:St+1-upper}.
\end{proof}
\end{lemma}

\subsection{The Upper Bound of $\E[S_{T+1}]$}
Recall the definition of $S_t$ in \Cref{eq:S-def}, we have
\begin{align*}
    S_{T+1} &= \sqrt{4+\sum_{t=1}^T (\ell_{t,i_t}^{\text{clip}})^2 \cdot (1-x_{t,i_t})^2 \cdot (K\log T)^{-1}} \\
    &\le \sqrt{4+\sum_{t=1}^T (\ell_{t,i_t}^{\text{clip}})^2 \cdot (K\log T)^{-1} }.
\end{align*}
Therefore, to control $\E[S_{T+1}]$, it suffices to control $\E[S]$ where $S$ is defined as follows:
\begin{align}\label{eq:S-def}
    S := \sqrt{4+\sum_{t=1}^T (\ell_{t,i_t}^{\text{clip}})^2 \cdot (K\log T)^{-1} }.
\end{align}

We give the following lemma on $\E[S_{T+1}]$:
\begin{lemma}
% \label{lemma:adv-S-bound}
    We have can bound the expectation of $S_{T+1}$ by
    \begin{align}
        \E[S_{T+1}] \leq 2 \cdot \sigma (K \log T)^{-\frac{1}{\alpha}} T^{\frac{1}{\alpha}}.
    \end{align}
\begin{proof}
    By clipping operation, we have
    \begin{align*}
        |\ell^{\text{clip}}_{t,i_t}| \leq C_{t,i_t} = S_t \cdot \frac{1}{4(1-x_{t,i_t})} \leq S_t \leq S_{T+1} \leq S.
    \end{align*}

    Therefore, we know
    \begin{align*}
        4 + \sum_{t=1}^T (\ell^{\text{clip}}_{t,i_t})^2\cdot (K \log T)^{-1} \leq \frac{1}{4}\sum_{t=1}^T |\ell_{t,i_t}|^\alpha \cdot S^{2-\alpha} \cdot (K \log T)^{-1},
    \end{align*}
    where the inequality is given by $S^2 \geq 16$, $|\ell^{\text{clip}}_{t,i_t}|\leq S$ and $|\ell^{\text{clip}}_{t,i_t}| \leq |\ell_{t,i_t}|$. Hence,
    \begin{align*}
        S^{\alpha} \leq \frac{4}{3}(K \log T)^{-1} \sum_{t=1}^T \lvert \ell_{t,i_t}\rvert^\alpha.
    \end{align*}
    
    Take expectation on both sides and use the convexity of mapping $x \mapsto x^{\alpha}$. We get
    \begin{align*}
        \E[S] &\leq \left(\frac{4}{3}\right)^{1/\alpha}(K \log T)^{-1/\alpha} \cdot \sigma \cdot T^{1/\alpha} \\
        &\leq 2(K \log T)^{-1/\alpha} \cdot \sigma \cdot T^{1/\alpha}.
    \end{align*}
    
    The conclusion follows from the fact that $S_{T+1}\le S$.
\end{proof}
\end{lemma}

\subsection{Bounding the sum of skipping errors}
\label{sec:adv-clipping}
% \yu{需要根据前面$\textsc{SkipErr}_t$部分的修改结果更改。主要需要更改的地方: 1. $S_t$定义; 2.$h_t$定义;}

\daiyan{到底是 clip 还是 skip？有点迷惑}

Recall the definition of $h_t = \ell_{t,i_t} - \ell^{\text{skip}}_{t,i_t} = \ell_{t,i_t}\cdot \mathbbm 1[\lvert \ell_{t,i_t} \rvert \ge C_{t,i_t}]$.
To control this skipping error, we perform a \textit{double-clipping} analysis. That is, in addition to the clipping threshold $C_{t,i}$, we additionally define a universal clipping threshold $M$ that is independent to both $t$ and $i$.
When analyzing, we first clip $\vl$ according to $M$. \daiyan{todo: need to motivate why we need to clip twice. I remember $M$ is used to ensure stopping time property?}
\yu{ 一个草稿: The key is to ensure an invariant clipping threshold $M$ serving as the stopping time of the increment of $S_t$ corresponding to time $t$. Then we can control that the number of $S_t \leq M$.}

Formally, we consider the following universal clipping threshold $M$:
\begin{equation*}
M:=\sigma (K\log T)^{-1/\alpha} T^{1/\alpha}.
\end{equation*}

We first perform a first clipping $\operatorname{Clip}(\ell_{t,i_t},M)$, which gives a \textit{universal} clipping error
\begin{equation*}
h_t^{\text{Univ}}:= \begin{cases}
\ell_{t,i_t} - M & \ell_{t,i_t} > M \\
0 & -M \le \ell_{t,i_t} \le M\\
\ell_{t,i_t} + M & \ell_{t,i_t} < -M
\end{cases}.
\end{equation*}

Then, we perform the secondary clipping $\operatorname{Clip}(\ell_{t,i_t},C_{t,i_t})$, as in \Cref{alg}.\yu{ 这句话什么意思来着 }

If $C_{t,i_t}\ge M$, then this clipping is ineffective. Otherwise, we get the following \textit{action-dependent} clipping error
\begin{equation*}
h_t^{\text{ActDep}} := \begin{cases}
h_t - h_t^{\text{Univ}} & C_{t,i_t} < M \\
0 & C_{t,i_t} \ge M
\end{cases}.
\end{equation*}


We have the following lemma
\begin{lemma}
% \label{lemma:adv-ht-sum}
Moreover, we have
\begin{align*}
    \E\left[\sum_{t=1}^T |h_t|\right] \leq 18\cdot  \sigma (K\log T)^{1-1/\alpha}T^{1/\alpha}\cdot \log \left((K \log T)^{-1/\alpha} \cdot \sigma \cdot T^{1/\alpha}\right)
\end{align*}
\begin{proof}
By above definitions, we trivially have $|h_t| \le |h_t^{\text{ActDep}}| + |h_t^{\text{Univ}}|$. Specifically, if $h^{\text{ActDep}}_t \ne 0$, we have $|h_t^{\text{ActDep}}| \leq M$ and $(\ell_{t,i_t}^{\text{clip}})^2 = C^2_{t,i_t}$ since $h_t \neq 0$. Therefore, we have
\begin{align*}
    S_{t+1}^2 = S_t^2 + C_{t,i_t}^2\cdot (1-x_{t,i_t})^2\cdot (K \log T)^{-1} = S_t^2 \left(1 + (K \log T)^{-1} / 4\right)
\end{align*}
as long as $h^{\text{ActDep}}_t \ne 0$.


Next we can bound $\sum_t \lvert h_t^{\text{ActDep}}\rvert$ and $\sum_t \lvert h_t^{\text{Univ}}\rvert$ separately. For $h_t^{\text{Univ}}$, we have
\begin{align*}
    \E[|h_t^{\text{Univ}}|] & \le \E[\lvert \ell_{t,i_t}\rvert\cdot \mathbbm 1[\lvert \ell_{t,i_t}\rvert \ge M]] \\
    & \le \E[|\ell_{t,i_t}|^\alpha]M^{1-\alpha} \\
    & \leq \sigma^\alpha M^{1-\alpha} \\
    & \le \sigma (K\log T)^{1-1/\alpha} T^{-1 + 1/\alpha}.
\end{align*}
Therefore,
$$
\sum_{t=1}^T \E[h_t^{\text{Univ}}] \le \sigma (K\log T)^{1-1/\alpha} T^{1/\alpha}.
$$

Since we have $S_{t+1}/S_t \geq \sqrt{1 + (K\log T)^{-1} / 4}$ for $t$ at which $h_t^{\text{ActDep}} \neq 0$. Thus the number of occurrences of non-zero $h_t^{\text{ActDep}}$'s is upper-bounded by $\lceil\log_{\sqrt{1+(K\log T)^{-1} / 4}} S_{T+1}\rceil$, and we have
\begin{align*}
    \E\left[\sum_{t=1}^T \lvert h_t^{\text{ActDep}}\rvert\right] & \le M\cdot \E[\log_{\sqrt{1+(K\log T)^{-1} / 4}} S_{T+1}] + M \\
    & = 2M \cdot \frac{\E[\log S_{T+1}]}{\log(1+(K\log T)^{-1} / 4)} + M. 
\end{align*}
Notice that we have $2x \geq \log(1+x^{-1})$ holding for $x \geq 1$. Therefore, by Jensen inequality, we have \jiatai{以后把下面的大O修掉}\yu{修了一下，请求检查}
\begin{align*}
    \E\left[\sum_{t=1}^T \lvert h_t^{\text{ActDep}}\rvert\right] & \le 16\cdot K\log T\cdot M \cdot \mathbb E[\log S_{T+1}] + M \\
 & \le 16\cdot K\log T \cdot M \cdot \log \E[S_{T+1}] + M \\
 & \le 16 \cdot \sigma (K\log T)^{1-1/\alpha}T^{1/\alpha}\cdot \log \left((K \log T)^{-1/\alpha} \cdot \sigma \cdot T^{1/\alpha}\right) + \sigma (K\log T)^{-1/\alpha} T^{1/\alpha}
 \\ &\leq 17 \cdot \sigma (K\log T)^{1-1/\alpha}T^{1/\alpha}\cdot \log \left((K \log T)^{-1/\alpha} \cdot \sigma \cdot T^{1/\alpha}\right)
% \\ & \leq \tilde \gO\left( \sigma K^{1-1/\alpha} (\log T)^{2-1/\alpha} T^{1/\alpha} \right).
\end{align*}

Combine these results together, we get
\begin{align*}
    \E\left[\sum_{t=1}^T |h_t|\right] & \leq \E\left[\sum_{t=1}^T |h_t^{\text{ActDep}}| + \sum_{t=1}^T |h_t^{\text{Univ}}|\right] \\
    & \leq 17 \cdot \sigma (K\log T)^{1-1/\alpha}T^{1/\alpha}\cdot \log \left((K \log T)^{-1/\alpha} \cdot \sigma \cdot T^{1/\alpha}\right) + \sigma (K\log T)^{1-1/\alpha} T^{-1 + 1/\alpha} 
    \\ &\leq 18 \cdot  \sigma (K\log T)^{1-1/\alpha}T^{1/\alpha}\cdot \log \left((K \log T)^{-1/\alpha} \cdot \sigma \cdot T^{1/\alpha}\right)
    % & = \tilde \gO(\sigma K^{1-1/\alpha}T^{1/\alpha}(\log T)^{2-1/\alpha}).
\end{align*}
\end{proof}
\end{lemma}



\subsection{The Main Result For Adversarial Case}

Equipped with the previous analysis, we can establish our main result of \Cref{alg} for adversarial setting.

\begin{theorem}\label{thm:regret-adv}
    For \Cref{alg}, under the adversarial case, we have
    \begin{align*}
        \gR_T \leq \gO\left(\sigma K^{1-1/\alpha}(\log T)^{2-1/\alpha}T^{1/\alpha}\cdot \log(\sigma K \log T)\right).
    \end{align*}
\begin{proof}
    Notice that by analysis in \Cref{sec:regret-skipping} and \Cref{sec:regret-ftrl}, we have
    \begin{align*}
        \gR_T  &\leq \sum_{t=1}^T \E\left[\textsc{FTRL}_t + \textsc{SkipErr}_t\right] + \sigma K \\
        &\leq  \E\left[\sum_{t=1}^T\textsc{Div}_t\right] + \E\left[ S_{T+1} \cdot K \log T \right] + \E\left[ \sum_{t=1}^T |h_t| \cdot \mathbbm{1}[i_t \neq i^\ast]\right].
    \end{align*}
    By \Cref{lemma:adv-bregman}, we have 
    \begin{align*}
        \gR_T \leq \left(8192(1 + \sqrt{2}) + 1\right) \cdot \E[S_{T+1} \cdot K \log T] + \E\left[ \sum_{t=1}^T |h_t| \right].
    \end{align*}
    Therefore, combining \Cref{lemma:adv-S-bound} and \Cref{lemma:adv-ht-sum}, we have
    \begin{align*}
        \gR_T &\leq 32770 \cdot \sigma (K \log T)^{1 - 1/\alpha} T^{1/\alpha} \\
        &\quad + 18 \cdot \sigma (K\log T)^{1-1/\alpha}T^{1/\alpha}\cdot \log \left((K \log T)^{-1/\alpha} \cdot \sigma \cdot T^{1/\alpha}\right) \\
        &= \gO\left(\sigma K^{1-1/\alpha}(\log T)^{2-1/\alpha}T^{1/\alpha}\cdot \log(\sigma K \log T)\right) \\
        &\leq \wt{\gO} \left( \sigma K^{1-1/\alpha}T^{1/\alpha}\cdot  \right)
    \end{align*}
\end{proof}
\end{theorem}


\section{Stochastic Regret Analysis}

\begin{lemma}
\label{lemma:At-bound}
    To bound the Bregman Divergence terms and the shifting terms in part (A), we have the following inequalities:
    \begin{align*}
        \E[\textsc{FTRL}_t] \leq 16386 \cdot S_t^{1-\alpha}\sigma^{\alpha}(1 - x_{t,i^\ast}).
    \end{align*}
\begin{proof}
First, for part (A), we can do the followings computation.
\begin{align*}
    \textsc{FTRL}_t & =\textsc{Div}_t + (\Psi_{t+1} - \Psi_t)(\wt{\vy}) - (\Psi_{t+1} - \Psi_t)(\vx_t) \\
\\    & \leq\textsc{Div}_t + \sum_{i\in[K]} (S_{t+1} - S_{t})(-\log(\wt{y}_i)) \\
    & \leq\textsc{Div}_t + (K\log T) \cdot \frac{S^2_{t+1} - S_t^2}{S_{t+1} + S_t} \\
    & \leq\textsc{Div}_t + \frac{(\ell_{t,i_t}^{\text{clip}})^2(1 - x_{t,i_t})^2}{2S_t},
\end{align*}
where the first inequality holds by $S_{t+1} \geq S_t$ and $\Psi_{t+1}(x) \geq \Psi_t(x)$, the second inequality holds by $-\log(\wt{y}_i) \leq -\log(1/T) = \log(T)$, and the third inequality holds by definition of $S_{t+1}$ in \Cref{eq:St-def} and $S_{t+1} \geq S_t$. 

Notice that by \Cref{lemma:bregman-bound}, we have
\begin{align}
\label{eq:Dt-upper-bound}
    \E[\textsc{Div}_t] \le 8192 \cdot S_t^{-1} \E\left[((\ell_{t,i_t}^{\text{skip}})^2(1 - x_{t,i_t})^2\right]  \leq 8192 \cdot S_t^{-1} \E\left[(\ell^{\text{clip}}_{t,i_t})^2(1 - x_{t,i_t})^2\right] 
\end{align}
By definition of $C_{t,i_t}$ in \Cref{eq:C-def}, we have
\begin{align*}
    \E[\textsc{FTRL}_t] &\leq 8193 \cdot S_t^{-1}\E\left[C_{t,i_t}^{2-\alpha}(1-x_{t,i_t})^{2-\alpha} |\ell_{t,i_t}|^{\alpha} (1 - x_{t,i_t})^{\alpha}\right] \\
    &\leq 8193 \cdot \frac{S_{t}^{1-\alpha}}{4^{2-\alpha}}\sigma^{\alpha}\sum_{i\in[K]}x_{t,i}(1 - x_{t,i})^\alpha 
\end{align*}
\yu{ 这里原本没有$\sigma$,我算这感觉需要？ } 

Notice that
\begin{align*}
    \sum_{i\in[K]}x_{t,i}(1 - x_{t,i})^\alpha &\leq \sum_{i \neq i^\ast} x_{t,i} + x_{t,i^\ast}(1 - x_{t,i^\ast}) \\
    &= (1 - x_{t,i^\ast}) + x_{t,i^\ast}(1 - x_{t,i^\ast}) \\
    &\leq 2(1 - x_{t,i^\ast})
\end{align*}

Therefore, we have
\begin{align*}
    \E[\textsc{FTRL}_t] \leq 16386 \cdot S_t^{1-\alpha}\sigma^{\alpha}(1 - x_{t,i^\ast})s.
\end{align*}
\end{proof}
\end{lemma}


Define 
\begin{align*}
    M := \inf \left\{ s > 0 : 16384 \cdot s^{1-\alpha} \sigma^\alpha \leq \Delta_{\min} / 4 \right\}
\end{align*}
Therefore, we have 
\begin{align*}
    M \leq \gO\left(\sigma^{\frac{\alpha}{\alpha - 1}}\Delta_{\min}^{-\frac{1}{\alpha - 1}} \right)
\end{align*}


We define the stopping time $\gT$ as
\begin{align*}
    \gT := \inf \left\{ t \geq 1 : S_t \geq M \right\} \wedge (T+1).
\end{align*}
Since we have $S_{t+1} \leq (1 + (K\log T)^{-1})S_t \leq 2S_t$ by \Cref{eq:}\yu{todo ref}, we have $S_{\gT}\leq 2M$. Moreover, we have the following lemmas

\begin{lemma}
\label{lemma:At-summation-previous}
    We have for given stopping time $\gT \leq T$, the sum of $\textsc{FTRL}_t$ can be bounded as follows
    \begin{align*}
        \E\left[\sum_{t=1}^\gT \textsc{FTRL}_t\right] \leq 16385 \cdot \E\left[S_{\gT + 1} \cdot (K \log T)\right].
    \end{align*}
\begin{proof}
Notice that we have
\begin{equation*}
    \textsc{FTRL}_t = \textsc{Div}_t + \left(\Psi_{t+1} - \Psi_t\right)(\wt\vy) - \left(\Psi_{t+1} - \Psi_t\right)(\vx_t)
\end{equation*}
By same approach as \Cref{lemma:shifting-terms}, we have
\begin{equation*}
    \sum_{t=1}^\gT \left(\Psi_{t+1} - \Psi_t\right)(\wt\vy) - \left(\Psi_{t+1} - \Psi_t\right)(\vx_t) \leq S_{\gT + 1} K \log T
\end{equation*}
holds for any $\gT \in [T]$. Moreover, by \Cref{eq:Dt-upper-bound}, we have
\begin{align*}
    \E[\textsc{Div}_t] &\leq 8192 \cdot \E[S_t^{-1} \cdot (\ell_{t,i_t}^{\text{clip}})^2(1 - x_{t,i_t})^2] \\
    &\leq 8192 \cdot \E[S_{t}^{-1} \cdot (K \log T) \cdot (S_{t+1}^2 - S_t^2)] \\
    &\leq 16384 \cdot \E[S_{t+1} - S_t] \cdot K \log T.
\end{align*}
Therefore, we have
\begin{equation*}
    \E\left[\sum_{t=1}^\gT \textsc{FTRL}_t\right] \leq 16385 \cdot \E\left[S_{\gT + 1} \cdot (K \log T)\right],
\end{equation*}
which finishes the proof.
\end{proof}
\end{lemma}


Therefore, we can decompose the sum of part (A)
\begin{align*}
    \E\left[\sum_{t=1}^T \textsc{FTRL}_t\right] &= \E\left[\sum_{t=1}^{\gT} \textsc{FTRL}_t\right] + \E\left[\sum_{t=\gT+1}^T \textsc{FTRL}_t \right] \\
    &\leq 16385 \cdot S_{\gT + 1} \cdot K\log T + \E\left[\sum_{t=\mathcal T}^{T} \textsc{FTRL}_t\right] \\
    &\leq 16385 \cdot S_{\gT + 1} \cdot K\log T + \E\left[ \sum_{t=\gT + 1}^T 16386 \cdot S_t^{1-\alpha} \sigma^\alpha (1 - x_{t,i^\ast}) \right] \\
    &\leq 16385 \cdot S_{\gT + 1} \cdot K\log T + \E\left[ \sum_{t=\gT + 1}^T 16386 \cdot M^{1-\alpha} \sigma^\alpha (1 - x_{t,i^\ast}) \right].
\end{align*}
where the first inequality is due to \Cref{lemma:At-summation-previous}, the second inequality is by \Cref{lemma:At-bound}, and the last inequality is due to the definition of stopping time $\gT$. Since $S_{\gT+1} \leq 2S_{\gT} \leq 4M$ and $16386\cdot M^{1-\alpha}\sigma^{\alpha} \leq \Delta_{\min}/4$, we have
\begin{align*}
    \E\left[\sum_{t=1}^T \textsc{FTRL}_t\right] & \leq65540 \cdot \left(M \cdot (K \log T) \right) + \frac{\Delta_{\min}}{4}\cdot \E\left[\sum_{t=\gT+1}^T (1 - x_{t,i^\ast})\right] \\
    & \leq\gO\left(K \sigma^{\frac{\alpha}{\alpha - 1}}\Delta_{\min}^{-\frac{1}{\alpha - 1}}\log T\right) + \frac{\gR_T}{4},
\end{align*}
where the last inequality is due to the definition of the cumulative regret.


\subsection{Bounding the Skipping Error Terms (Part $\textsc{SkipErr}$)}
For part $(B)$, we have %\jiatai{我把最开始你多打、一路抄写到这里的indicator去掉了}
\begin{align*}
    \textsc{SkipErr}_t & =\sum_{i \in [K]}(x_{t,i} - y_i) \cdot (\ell_{t,i} - \ell^{\prime}_{t,i})
\end{align*}


We consider the same definition of $h^{\text{ActDep}}_t$ and $h^{\text{Univ}}_t$ as the analysis in adversarial case in \Cref{sec:adv-clipping}. For readability, we repeat the definition here. Consider the truncation constant $M$ defined as
\begin{align*}
    M := \inf \left\{ s > 0 : 16384 \cdot s^{1-\alpha} \sigma^\alpha \leq \Delta_{\min} / 4 \right\}
\end{align*}
Then consider $h_t^{\text{ActDep}}$ and $h_t^{\text{Univ}}$:
\begin{align*}
h^{\text{ActDep}}_t :& =\begin{cases}
h_t - h^{\text{Univ}}_t & C_{t,i_t} < M \\
0 & C_{t,i_t} \ge M
\end{cases}, \\
h^{\text{Univ}}_t :& =\begin{cases}
\ell_{t,i_t} - M & \ell_{t,i_t} > M \\
0 & -M \le \ell_{t,i_t} \le M\\
\ell_{t,i_t} + M & \ell_{t,i_t} < -M
\end{cases}.
\end{align*}
By \Cref{eq:Bt-bound-by-ht}, we have %\jiatai{我改了一下，你看看}
\begin{align*}
    \E[\textsc{SkipErr}_t] \leq \E\left[\left|h_t\right|\cdot \mathbbm 1[i_t \ne i^\ast]\right] \leq \E\left[\left|h_t^{\text{ActDep}}\right|\cdot \mathbbm 1[i_t \ne i^\ast]\right] + \E\left[\left|h_t^{\text{Univ}}\right|\cdot \mathbbm 1[i_t \ne i^\ast] \right].
\end{align*}
Specifically, if $h_t^{\text{ActDep}} \neq 0$, we have 
\begin{align*}
    \left| h_t^{\text{ActDep}} \right| \leq \max \left( M - C_{t,i_t}, 0\right) \leq M.
\end{align*}
Moreover, we have $h_t \neq 0$, which implies that $\ell^{\prime}_{t,i_t} = 0$, $\ell^{\prime\prime2}_{t,i_t} = C_{t,i_t}$, and 
\begin{align*}
    S_{t+1}^2 = S_t^2 + C_{t,i_t}^2 \cdot (1 - x_{t,i_t})^2 \cdot (K \log T)^{-1} = S_t^2 \left(1 + (4K \log T)^{-1}\right).
\end{align*}
If $S_t \geq M$, we have $C_{t,i} = \frac{S_t}{4(1 - x_{t,i})} \geq M$ holds for every $i \in [K]$, showing that $h_t^{\text{ActDep}} = 0$. Thus the number of occurrences of non-zero $h_t^{\text{ActDep}}$'s is upper-bounded by $\lceil\log_{\sqrt{1+(4K\log T)^{-1}}} M\rceil$, and we have
\begin{align*}
    \E\left[\sum_{t=1}^T \left\lvert h_t^{\text{ActDep}}\right\rvert \right] & \le M\cdot \E[\log_{\sqrt{1+(K\log T)^{-1} / 4}} M] \\
    & = 2M \cdot \frac{\log M}{\log(1+(4K\log T)^{-1})} \\
    &\leq \gO\left(K\log T \cdot M \log M\right) \\
    &\leq \gO\left(K \log T \cdot \sigma^{ \frac{\alpha}{\alpha - 1} }\Delta_{\min}^{ -\frac{1}{\alpha - 1} }\cdot \log (1/\sigma\Delta_{\min})\right)
\end{align*}
For $h_t^{\text{Univ}}$, we have %\jiatai{下面LHS期望里面加上$\mathbbm 1[i_t \ne i^\ast]$因子，然后可以chain rule先弄出$(1-x_{t,i^\ast})$，剩下的条件期望统一放成$\sigma^\alpha \cdot M^{1-\alpha}$}
\begin{align*}
    \E\left[\sum_{t=1}^T |h_t^{\text{Univ}}|\cdot \mathbbm{1}[i_t \neq i^\ast]\right] &\leq  \sum_{t=1}^T \E[ \mathbbm{1}[i_t \neq i^\ast] \cdot \mathbbm{1}[|\ell_{t,i_t}|>M]\left|\ell_{t,i_t} - M\right|] \\
    &\leq \sum_{t=1}^T \E\left[\mathbbm{1}[i_t \neq i^\ast] \cdot |\ell_{t,i_t}|^\alpha\right]M^{1-\alpha} \\
    &\leq \sum_{t = 1}^T (1 - x_{t,i^\ast}) \sigma^\alpha M^{1-\alpha} \\
    &\leq \frac{\Delta_{\min}}{4}\sum_{t=1}^T (1 - x_{t,i^\ast}) \\
    &\leq \frac{\gR_T}{4}
\end{align*}

Therefore, we have

\begin{align*}
    \E\left[ \sum_{t=1}^T \textsc{SkipErr}_t \right] \leq \gO\left( K \log T \cdot \sigma^{ \frac{\alpha}{\alpha - 1}} \Delta_{\min}^{-\frac{1}{\alpha - 1}} \cdot \log(1 / \sigma \Delta_{\min})  \right) + \frac{1}{4}
    \gR_T
\end{align*}

\subsection{The Main Result For Stochastic Case}

Combine the results together, we have
\begin{theorem}
\label{thm:regret-sto}
  For \Cref{alg}, under the stochastic settings, we have
    \begin{equation*}
        \gR_T \leq \gO\left(K\log T \sigma^{\frac{\alpha}{\alpha - 1}} \Delta_{\min}^{-\frac{1}{\alpha - 1}} \cdot \log(1/\sigma\Delta_{\min})\right)
    \end{equation*}
\begin{proof}
    Combining the results in previous sections, we have
    \begin{align*}
        \gR_T &\le \E\left[\sum_{t=1}^T \textsc{FTRL}_t + \textsc{SkipErr}_t\right] + \sigma K \\
        &\leq \gO\left(K\log T \sigma^{\frac{\alpha}{\alpha - 1}} \Delta_{\min}^{-\frac{1}{\alpha - 1}} \cdot \log(1/\sigma\Delta_{\min})\right) + \frac{1}{2}\gR_T,
    \end{align*}
    which implies that
    \begin{equation*}
        \gR_T \leq \gO\left(K\log T \sigma^{\frac{\alpha}{\alpha - 1}} \Delta_{\min}^{-\frac{1}{\alpha - 1}} \cdot \log(1/\sigma\Delta_{\min})\right).
    \end{equation*}
    in stochastic settings. 
\end{proof}
\end{theorem}
